Disconnected Matchings

In 2005, Goddard, Hedetniemi, Hedetniemi and Laskar [Generalized subgraph-restricted matchings in graphs, Discrete Mathematics, 293 (2005) 129 - 138] asked the computational complexity of determining the maximum cardinality of a matching whose vertex set induces a disconnected graph. In this paper we answer this question. In fact, we consider the generalized problem of finding $c$-disconnected matchings; such matchings are ones whose vertex sets induce subgraphs with at least $c$ connected components. We show that, for every fixed $c \geq 2$, this problem is NP-complete even if we restrict the input to bounded diameter bipartite graphs, while can be solved in polynomial time if $c = 1$. For the case when $c$ is part of the input, we show that the problem is NP-complete for chordal graphs, while being solvable in polynomial time for interval graphs. Finally, we explore the parameterized complexity of the problem. We present an FPT algorithm under the treewidth parameterization, and an XP algorithm for graphs with a polynomial number of minimal separators when parameterized by $c$. We complement these results by showing that, unless NP $\subseteq$ coNP/poly, the related Induced Matching problem does not admit a polynomial kernel when parameterized by vertex cover and size of the matching nor when parameterized by vertex deletion distance to clique and size of the matching. As for Connected Matching, we show how to obtain a maximum connected matching in linear time given an arbitrary maximum matching in the input.

==> appendices.tex <==
\newpage
\setcounter{section}{0}
\renewcommand\thesection{\Alph{section}}
\section*{Appendix}

\section{Proof of Theorem \ref{teo:c-disc-induced-np-complete}}\label{app:c-disc-induced-np-complete}
The input data set for the {\sc $k$-Induced Matching} is a subset of the possible inputs from {\sc $c$-Disconnected Matching}, since these problems are equivalent when using $c = k$. Therefore, the {\sc $c$-Disconnected Matching} is NP-complete, because it is an extension of {\sc $k$-Induced matching}. Such reduction does not alter the input $G$ graph and, therefore, its properties are preserved when considering with the problem {\sc $c$-Disconnected Matching}.


\section{Proof of Theorem \ref{teo:emp-1-desc}}\label{app:emp-1-desc}
Solving the {\sc $1$-Disconnected Matching} decision problem is equivalent to ask if the answer to {\sc Maximum Matching} is $\geq k$. This equivalency is true because $G[M]$ can have any number of connected component in both. Therefore, {\sc $1$-Disconnected Matching} is in {\P} and can be solved in the same complexity of {\sc Maximum Matching}, which is $\bigO{|E|\sqrt{|V|}}$ \cite{vazirani}.

\section{Proof of Theorem \ref{teo:connected-matching-complexity}}\label{app:connected-matching-complexity}
The proof of Theorem \ref{teo:connected-matching-complexity} is given below by the Algorithm \ref{EmpConexoGeralNPonderado} and its proofs of complexity and correctness.

The idea of the algorithm, based on the the equality $\beta = \beta_c$\cite{GODDARD2005129}, is that, given a maximum matching $M$, it is possible to build a connected matching with the same cardinality just by swapping edges of $M$, without changing its cardinality.

We now describe how the edge swap operation can be done. Let $M$ be a maximum matching such that $G[M]$ is disconnected and $r$ any $M$-saturated vertex. Let $C_r$ be the connected component of $G[M]$ that contains $r$ and $W = \{w \mid w \in N(v) \setminus V(C_r) , \forall v \in C_r \} $, that is, $W$ is the set of vertices not in $V(C_r)$ but adjacent to some vertex of $V(C_r)$. Observe that, in $G$, there is a saturated vertex $u \notin V(C_r)$ adjacent to some vertex $w \in W$. Therefore, it is possible to increase the connected component $C_r$ by removing the saturated edge of $u$ from $M$ and adding the edge $uw$. This procedure can be done until $G[M]$ is connected.

The algorithm uses two queues, $Q_s$ and $Q_n$, to store saturated and not saturated vertices by $M$, respectively, and a set $C$, to which vertices of $C_r$ or new vertices are added. The main loop includes at least one vertex to $C$ at each iteration and is divided into two other auxiliary loops. The first auxiliary loop, executes \Call{expand}{$v$} for each vertex $v$ of $Q_s$, analyses $N(v)$ and appropriately adds to the queue each vertex in that neighborhood that has not yet been inserted in the queue. The second auxiliary loop executes the function \Call{tryToConnect}{$v$} for each vertex $v$ of $Q_n$. If there exists $w \in N(v) \setminus C$, then $w$ must be saturated by an edge $wu$, so the edge swap operation is performed in $M$, removing the edge $wu$ and adding the edge $vw$.

\begin{nofloatalgorithmic}[1]{Maximum Connected Matching}{EmpConexoGeralNPonderado}
    \Statex   
    \Function{Expand}{Vertex: $v$}
      \For{$w \in N(v)\setminus C$}
          	\If{$w$ is $M$-saturated}
              	\Let{$C$}{$C \cup \{w\}$}
              	\State Insert $w$ in $Q_s$
            \ElsIf{$w \notin W$}
                    \Let{$W$}{$W \cup \{w\}$}
                    \State Insert $w$ in $Q_n$
          	\EndIf
      \EndFor
    \EndFunction
    \State
    
    \Function{tryToConnect}{Vertex: $v$}
      \If{$\exists w \in N(v) \setminus C$}
          	\Let{$u$}{vertex matched with $w$ in $M$}
          	\Let{$M$}{$M \setminus \{uw\} \cup \{vw\}$}
          	\Let{$C$}{$C \cup \{v, w\}$}
          	\Let{$W$}{$W \setminus \{v\}$}
          	\State Insert $v$ and $w$ in $Q_s$
      \EndIf
    \EndFunction
    \State
    \State \#Input:
    $G$: Graph, 
    $M$: Maximum matching of $G$
    \State
    \LetVertical{$W$}{$ \emptyset$; \ \ }
    \LetVertical{$Q_s$}{$ \emptyset$; \ \ }
    \LetVertical{$Q_n$}{$ \emptyset$;}

        \Let{$r$}{any $M$-saturated vertex}
        \Let{$C$}{$ \{r\}$}
        
        \State Insere $r$ em $Q_s$
        \While{$|C| < |M|*2$}
        
            \While{$Q_s$ is not empty}
                \Let{$v$}{vertex removed from the front of $Q_s$}
                \State \Call{Expand}{$v$}
            \EndWhile
            \While{$Q_n$ is not empty}
                \Let{$v$}{vertex removed from the front of $Q_n$}
                \State \Call{tryToConnect}{$v$}
            \EndWhile
        \EndWhile
        \State return $M$
\end{nofloatalgorithmic}

The Figure~\ref{fig:example-connected} illustrates two maximum matchings for a graph. On the left, an arbitrary maximum matching that can be used as input of Algorithm $1$, generating the maximum connected matching on the right.

%This matching can be obtained by the Algorithm~\ref{GeneralConexoNPweighted} if we choose, for example, $c$ as the initial vertex. It is placed in the queue $Q_s$ and in $C$. The procedure $\Call{Expand}{c}$ adds the vertices $g$ and $h$ to the queue $Q_s$ and to the set $C$. It also adds the vertex $a$ to the queue $Q_n$ and to the set $W$. Next, the vertex $a$ of the queue $Q_n$ is processed by the procedure $\Call{tryToConnect}{a}$. The vertex $b \notin N(a) \setminus C$ is found. Then, in $M$ the edge $(b,e)$ is removed and the $(a,b)$ inserted. The vertices $a$ and $b$ are placed in $C$. In the remainder of the algorithm no further changes in $M$ are made and the maximum connected match is obtained.

\begin{lemma}\label{teo:EmpConexoGeralNPond}
Algorithm \ref{EmpConexoGeralNPonderado} runs in $\bigO{|V|+|E|}$.
\end{lemma}
\begin{proof}

The main loop runs until the connected component has the desired size. At the beginning of each iteration, we know that $G[M]$ is not connected yet because of the loop stopping condition. Since, at the end of the loop, at least one vertex is added to $C$, the number of iterations is $\bigO{|V|}$. The sets $C$ and $W$ act as markers for the queues, so each vertex $v \in V(G)$ can only be processed at most once in the functions $\Call{expand}{v} $ and $\Call{tryToConnect}{v}$. Note that the execution of these functions analyses the neighborhood of $v$ and, therefore, has linear complexity to the degree of $v$. Hence, the complete algorithm has linear complexity with respect to vertices and edges.
\end{proof}

Note that, to use Algorithm \ref{EmpConexoGeralNPonderado}, it is necessary to have calculated a maximum matching before. To obtain a maximum matching, an algorithm with complexity $\bigO{|E|\sqrt{|V|}}$ is known\cite{vazirani}. Therefore, this complexity is the same as the { \sc Maximum Connected Matching}.

%That is, the { \sc Maximum Connected Matching } problem has a polynomial solution and its complexity is restricted to the { \sc Maximum Matching} complexity. 

Some classes, such as trees and block graphs, have linear time algorithms for the { \sc Maximum Matching}\cite{BrunoMasquio:2019:TeseMestrado}\footnote{Savage, C.: Maximum matchings and trees. Information Processing Letters 10(4),
202 - 205 (1980). https://doi.org/10.1016/0020-0190(80)90140-4}. Hence, for these classes, the existence of Algorithm \ref{EmpConexoGeralNPonderado} shows that { \sc Maximum Connected Matching } is linear as well.

The Table \ref{tab:example-connected} shows an example of the execution of the Algorithm \ref{EmpConexoGeralNPonderado} with the input matching $M = \{cg, hj, be, di\}$. The vertex $c$ was chosen as the initial. Each line represents the state of the variables after the execution of the function specified in the first column. The lines are in ascending order according to when the functions are executed.

\begin{figure}%
        \centering
        \subfloat[]{{\includegraphics[width=0.35\textwidth]{images/example-connected-1} }}
        \hspace{0.15\textwidth}
        \subfloat[]{{\includegraphics[width=0.35\textwidth]{images/example-connected-2} }}
        
        \caption{Maximum matching(a) and maximum connected matching(b).}%
        \label{fig:example-connected}
\end{figure}

\begin{table}\label{tab:ex-alg-connected}
\caption{ {\small Example of variable contents from an execution of the Algorithm~\ref{EmpConexoGeralNPonderado} }}
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline
Função executada & $C$ & $W$ & $Q_s$ & $Q_n$ & $M$\\
\hline
%Inicialização & \{c\}    & \{\}                              & \{c\} 		& \{\} 		& \{(c,g), (h,j), (b,e), (d,i)\} \\
$\Call{expand}{c}$ & \{c, g, h\}     & \{a\}                      & \{g,h\} 	& \{a\} 		& \{cg, hj, be, di\} \\
$\Call{expand}{g}$ & \{c, g, h\}     & \{a\}                      & \{h\}  	& \{a\} 		& \{cg, hj, be, di\} \\
$\Call{expand}{h}$ & \{c, g, h, j\}     & \{a\}                   & \{j\}  	& \{a\} 		& \{cg, hj, be, di\} \\
$\Call{expand}{j}$ & \{c, g, h, j\}     & \{a\}                   & \{\}  		& \{a\} 		& \{cg, hj, be, di\} \\
$\Call{tryToConnect}{a}$ & \{c, g, h, j, a, b\}    & \{\}               & \{a,b\}  	& \{\} 		& \{cg, hj, ab, di\} \\
$\Call{expand}{a}$ & \{c, g, h, j, a, b, d\}     & \{\}           & \{b,d\}  	& \{\} 		& \{cg, hj, ab, di\} \\
$\Call{expand}{b}$ & \{c, g, h, j, a, b, d\}     & \{e\}          & \{d\}  	& \{e\} 		& \{cg, hj, ab, di\} \\
$\Call{expand}{d}$ & \{c, g, h, j, a, b, d, i\}     & \{e\}       & \{i\}  	& \{e\} 		& \{cg, hj, ab, di\} \\
$\Call{expand}{i}$ & \{c, g, h, j, a, b, d, i\}     & \{e\}       & \{\}  		& \{e\} 		& \{cg, hj, ab, di\} \\
$\Call{tryToConnect}{e}$ & \{c, g, h, j, a, b, d, i\}     & \{e\}       & \{\}  		& \{\} 		& \{cg, hj, ab, di\} \\
\hline
\end{tabular}\label{tab:example-connected}
\end{table}

\section{Proof of Lemma \ref{lemma:H1H2matched}}
We denote $A$ by the subgraph induced by the vertices of $V(G) \setminus V(H_1) \setminus V(H_2)$. Note that $A$ is exactly the subgraph induced by the vertex set of $B_i$, $i \in \{ 1,\ldots,m \}$.

In order to obtain $M$ with cardinality $k$, it is necessary that $2k \geq 2\cdot(12m) = 24m$ vertices are saturated by $M$. Note that $|V(A)| = 18m$. Since we are looking for a $k$ cardinality matching, then, even if all the vertices of $A$ were saturated, we would have, at most, $18m$ vertices. Therefore, for $M$ to saturate $2k$ vertices, we need to use vertices of $V(H_1) \cup V(H_2)$. Note that, similarly, if vertices of $A$ and only one of the subgraphs $H_1$ or $H_2$, $|V(H_1)| = |V(H_2)| = 6m$, we will have a maximum of $24m$ vertices, however, the matching would be perfect in the subgraph and, therefore, connected. Thus, it is necessary that there are at least two vertices $h_1 \in V(H_1)$ and $h_2 \in V(H_2)$ saturated by $M$.

\section{Proof of Lemma \ref{lemma:duasComponentesConexas}}
From Lemma \ref{lemma:H1H2matched}, we know that $M$ saturates $h_1 \in V(H_1)$ and $h_2 \in V(H_2)$ by two edges, $(h_1, v_1)$ e $(h_2, v_2)$. Note that, due to the graph structure, every edge $e$ saturated by $M$ is incident to at least one vertex of $V(G) \setminus \{ l_{i7}, l_{i8}, l_{i9}, r_{i7}, r_{i8}, r_{i9} \}$, $i \in \{ 1,\ldots,m \}$, as every edge of the graph has this property. Then, one end of $e$ is adjacent to any of the vertices in $\{ h_1, v_1, h_2, v_2 \}$. Therefore, $G[M]$ has exactly two connected components $C_1$ and $C_2$ such that $h_1 \in V(C_1)$ and $h_2 \in V(C_2)$.

\section{Proof of Lemma \ref{lemma:6-arestas}}

%From Lemma \ref{lemma:12VerticesSaturados}, we show that any separator between the two connected components of $G[M]$ can be partitioned into $m$ smaller $h_1-h_2$ separators, $h_1 \in V(H_1)$ and $h_2 \in V(H_2)$, one for each clause subgraph.

Let $h_1 \in V (H_1)$ and $h_2 \in V(H_2)$, $M$ be a $2$-disconnected matching in $G$, and $S_i$ be a $h_1-h_2$ minimal separator in $G_i^+$. For the rest of the proof, we use $S_i$ separators with cardinality $6$, so that all $12$ vertices of $V(B_i) \setminus S_i$ will be saturated by $M$. We prove that there are only $3$ separators of this type, due to the following properties.

\begin{enumerate}
    \item The vertices $l_{ij}$, $j \in \{ 7,8,9 \}$, are never part of $S_i$, because they are not part of any minimum path between $h_1$ e $h_2$.
    \item The vertex pairs $l_{ij}$ e $r_{i(j+3)}$ cannot be saturated simultaneously. Thus, $S_i$ contains exactly one of these two vertices.
    \item The vertex $l_{ij}$ cannot be saturated simultaneously with $r_{iq}$ or $r_{it}$, $j,q,t \in \{ 1,2,3 \}$, distincts.
    \item If there are two saturated vertices $l_{ij}$ e $l_{iq}$, then the four vertices $r_{ij}$, $r_{iq}$, $r_{it}$ and $r_{i7}$ can not be saturated, $j,q,t \in \{ 1,2,3 \}$, distinct.
    \item The number of saturated vertices of $\{ l_{i8}, l_{i9} \}$ must be less or equal to the number of saturated vertices of $\{ l_{i4},l_{i5},l_{i6} \}$.
\end{enumerate}

Note that the properties are similar for vertices of type $l$ and $r$. Thus, there are another $5$ properties analogous to those listed for $r$ vertices.

%These properties serve as the basis for the Lemma \ref{lemma:12VerticesSaturados}.

\begin{lemma}\label{lemma:12VerticesSaturados}
If $M$ is a disconnected matching with cardinality $\geq k$, $B_i$ is a clause subgraph and $W_i$ the $M$-saturated vertex set of $B_i$, then $W_i$ has cardinality $12$ and is one of the three sets indicated in the Table \ref{tab:separadoresBi}.
\end{lemma}
\begin{proof}
Let $S_i$ be a $h_1-h_2$ separator, $h_1 \in V(H_1)$, $h_2 \in V(H_2)$. Consider $W_i$ the set of vertices in $V(B_i) \setminus S_i$ that could possibly be saturated by $M$. For Property $1$, we can deduce that, for the set $R = \{ l_{i7},l_{i8},l_{i9},r_{i7},r_{i8},r_{i9} \}$, it is true that $S_i \cap R = \emptyset$ and $R \subseteq W_i$. Given the Property $2$, we can see that $| S_i | \geq 6$. With that, $| W_i | \leq 12 $, that is, the largest number of saturated vertices in a clause subgraph is $12$. Next, we'll show that there are only $3$ separators and $W_i$ sets of that type. Note that, for Property $4$, if we want to get a minimal separator $S_i$ such that $|W_i| = 12$, there can only be a single saturated vertex $l_{ij}$, $j \in \{ 1,2,3 \}$. In addition, for $r_{i7}$ to be in $W_i$, a vertex $r_{it}$, $t \in \{ 1,2,3 \}$ must be in $W_i$ as well. For Property $3$, the only possibility for this to occur is if $j = t$. Thus, the vertices $l_{i (j + 3)} $ and $r_{i (j + 3)}$ cannot belong to $W_i$. In addition, for Property $5$, for $l_{i8}$ and $l_{i9}$ to be in $W_i$, two vertices $l_{i (q + 3)}$ for $q \in \{ 1,2,3 \}$ are in $W_i$ as well. The only possibility of this occurring is if $q \neq j$. The same is true for the vertices $r_{i (q + 3)}$. Finally, we can define the set described as $W_i =$ $\{ l_{ij}, r_{ij}, l_{i(q+3)}, r_{i(q+3)}, l_{i(t+3)}, r_{i(t+3)}$ $|$ $ j,q,t \in \{ 1,2,3 \}, \text{distinct} \}$ $\cup$ $\{ l_{ij}, r_{ij} \mid j \in \{ 7,8,9 \} \}$. Therefore, there are only $3$ possibilities for the set $W_i$, which are present in Table \ref{tab:separadoresBi} and in Figure \ref{fig:separadoresBi}.
\end{proof}


\begin{table}
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
  $h_1-h_2$ separator of $G_i^+$ & Possibly saturated remaining vertices \\ 
 \hline
    $\{ l_{i2}, l_{i3}, l_{i4}, r_{i2}, r_{i3}, r_{i4} \}$ & $\{ l_{i1}, l_{i5}, l_{i6}, l_{i7}, l_{i8}, l_{i9}, r_{i1}, r_{i5}, r_{i6}, r_{i7}, r_{i8}, r_{i9}\}$ \\
    
    $\{ l_{i1}, l_{i3}, l_{i5}, r_{i1}, r_{i3}, r_{i5} \}$ & $\{ l_{i2}, l_{i4}, l_{i6}, l_{i7}, l_{i8}, l_{i9}, r_{i2}, r_{i4}, r_{i6}, r_{i7}, r_{i8}, r_{i9}\}$ \\
    
    $\{ l_{i1}, l_{i2}, l_{i6}, r_{i1}, r_{i2}, r_{i6} \}$ & $\{ l_{i3}, l_{i4}, l_{i5}, l_{i7}, l_{i8}, l_{i9}, r_{i3}, r_{i4}, r_{i5}, r_{i7}, r_{i8}, r_{i9}\}$ \\
 \hline
\end{tabular}
\end{center}
\caption{Some $h_1-h_2$ minimal separators in a subgraph $G_i^+$ and the respective remaining sets of vertices, which can be saturated} \label{tab:separadoresBi}
\end{table}


Analyzing the subgraph $G_i^+$ and the sets of vertices that can be saturated by the Lemma \ref{lemma:12VerticesSaturados}, we can define the edges that are used.

Note that the only possible edge sets can be generated from the following process. For each subgraph $B_i$, generate a matching with cardinality $6$ where each edge is disjointly incident to one of the vertices $\{ l_{i7}, l_{i8}, l_{i9}, r_{i7}, r_{i8}, r_{i9} \}$. Since $H_1$ and $H_2$ are complete bipartite subgraphs with the same number of vertices for each partition, it is possible to generate a matching by saturating all vertices, with $6m$ edges. At the end of the process, we have the $12m$ edges.

Therefore, the $12$ saturated vertices of $B_i$ indicated in Lemma \ref{lemma:12VerticesSaturados} corresponds to $6$ edges in $G[V(B_i)]$.

%This conclusion is related to the following Corollary.

%Note that, a disconnected matching with cardinality $12m$ is a maximum disconnected matching.

\begin{figure}%
        \centering
        \subfloat[]{{\includesvg[width=6.75cm]{images/svg/gadget-clausula-separadores-1-indices-invertidos} }}
        \subfloat[]{{\includesvg[width=6.75cm]{images/svg/gadget-clausula-separadores-2-indices-invertidos} }}
        
        \subfloat[]{{\includesvg[width=6.7cm]{images/svg/gadget-clausula-separadores-3-indices-invertidos} }}
        \caption{Subgraph $B_i$ with, in bold, the three sets of vertices possibly saturated with cardinality $12$ from Table \ref{tab:separadoresBi}.}%
        \label{fig:separadoresBi}
\end{figure}


\section{Proof of Lemma \ref{lemma:NPHardVolta}}
For this Lemma to be true, using the $R$ assignments, each clause in $I$ must have exactly one true literal and each variable must have the same assignment in all clauses. As was deduced in the Lemma \ref{lemma:12VerticesSaturados}, in fact, given $i$, $l_ {ij}$ is saturated only for a single $j$, $j \in \{ 1,2,3 \}$, $i \in \{ 1,\ldots,m \}$. So we have a single true literal. We now show that the assignment of the variable is consistent across all clauses. By contradiction, assume this to be false, then in $R$ there are two literals, $x$ and $y$, for the same variable, and one of the following two possibilities occurs. Consider $x$ o $q$-th literal of $c_i$ and $y$ o $t$-th literal of $c_j$. Either there is one negation between $x$ and $y$ or $x$ and $y$ have the same sign. In the first possibility, as we assumed that $x$ and $y$ have different assignments, then either $r_{iq}$ and $l_{jt}$ are saturated simultaneously or $ l_{i (q + 3)}$ and $r_{j (t + 3)} $ are. Note that $c_i$ and $c_j$ have variables with opposite literals, which means that the constructed graph has the edges $r_{iq}l_{jt}$ and $l_{i(q + 3)}r_{j(t+3)}$. Therefore, by the Lemma \ref{lemma:H1H2matched}, $G[M]$ would be connected, which is a contradiction. In the second possibility, $x$ and $y$ have the same sign. So either $l_{i (q + 3)}$ and $r_{jt}$ are saturated simultaneously or $r_{iq}$ and $l_{j (t + 3)}$ are. There are also edges between these pairs of vertices and, also by Lemma \ref{lemma:H1H2matched}, it is a contradiction. Therefore, $R$ solves {\sc One-in-three 3SAT}.

\section{Proof of Lemma \ref{lemma:NPHardIda}}
In the procedure described, we are saturating $6$ edges for each clause in (I), and $6m$ edges in (II). Then, $M$ has $12m$ edges. We need to show now that $M$ is disconnected. It is necessary and sufficient showing that there are not two adjacent vertices $l$ and $r$ saturated. Edges between vertices of the same clause subgraph are generated in (I) and we observe that there are no two adjacent saturated vertices of this type, since the saturated vertices are those described in Lemma \ref{lemma:12VerticesSaturados}. The vertices incident to the edges between different clause subgraphs can not be simultaneously saturated, as they would represent variables and their negations as true. Therefore, $M$ is disconnected and $|M| = 12m$.

\section{Proof of Lemma \ref{lemma:disc-match-np-c-diameter}}
Let's show that a $2$-disconnected matching $M$ in $G'$, $|M| \geq 12m$, saturates only vertices of $V(G)$ and, therefore, $M$ is also a $2$-disconnected matching in $G$. With this purpose, we demonstrate that the vertices $w_1$ and $w_2$ are not part of $M$. Let's assume that $w_1$ is saturated and $w_1 \in C_1$. Note that, since $G'$ is bipartite, then every edge $e \in E(G')$ has one endpoint at $V(V_1')$ and other at $V(V_2')$. Therefore, the edge $e$, if saturated, would be at $C_1$. 
Thereby, $M$ would not be $2$-disconnected, which is a contradiction. This shows that $w_1$ is not saturated. The argument is analogous to $w_2$. Thus, if $M$ is a $2$-disconnected matching in $G'$, $|M| \geq 12m$, so it's also in $G$. As we have already described the structure of such matchings in $G$ in Lemmas \ref{lemma:H1H2matched}, \ref{lemma:duasComponentesConexas} and \ref{lemma:6-arestas}, this transformation can also be used to solve the {\sc One-in-three 3SAT} problem.

\section{Proof of Theorem \ref{theo:npcomplete}}
Let $G = (V_1 \cup V_2, E)$ be a graph generated from the transformation of Section \ref{subsec:transformacaoEntrada}. Let's show that this graph is bipartite. Note that the bipartition $V_1$ of $G$ can be defined by $V_1 = \{ l_{iq} $ $|$ $i \in \{ 1,\ldots,m \}, q \in \{ 1,\ldots,6 \} \}$ $\cup$ $ \{ r_{iq} $ $|$ $i \in \{ 1,\ldots,m \}, q \in \{7,8,9\} \}$ $\cup$ $\{ u_1, u_3 $ $|$ $u_1 \in V(U_1), u_3 \in V(U_3) \}$.

Next, we prove that the problem is in {\NP} and {\NPH}. Let $M$ be a disconnected matching with cardinality $\geq k$. The matching $M$ serves as a certificate for the problem's {\YES} answer, checking its cardinality and if $G[M]$ is disconnected, which can be done in polynomial time. So, the problem is in {\NP}. According to the transformations between {\sc $2$-Disconnected Matching} and {\sc One-in-Three 3SAT} solutions described in Lemmas \ref{lemma:NPHardIda} and \ref{lemma:NPHardVolta}, the {\sc One-in-three 3SAT} problem, which is {\NPc}, can be reduced to {\sc $2$-Disconnected Matching} using a diameter $3$ bipartite graph. Therefore, {\sc $2$-Disconnected Matching} is {\NPH}. Thereby, we prove that {\sc $2$-Disconnected Matching} is {\NPc} even for diameter $3$ bipartite graphs.


\begin{comment}
\section{Notes about Corollaries \ref{coro:dicothomyBipartite} and \ref{coro:dicothomyGeneral}}

We show some statements about the diameters used in Colloraries \ref{coro:dicothomyBipartite} and \ref{coro:dicothomyGeneral}.

%Observe que um grafo com diâmetro $d \leq 2$, se conexo, ou é um grafo vazio ou é um grafo bipartido completo ou é um grafo completo. Para os três casos, a resposta para o {\sc Emparelhamento Desconexo} é sempre NÃO.

Note that a graph with diameter $d \leq 2$, if connected, is either an empty graph or a complete bipartite graph or a complete graph. For all three cases, the answer to {\sc $2$-Disconnected Matching} is always \NOi.

%Em contrapartida, se o grafo é desconexo, há duas possibilidades. Caso ele não possua pelo menos uma componente conexa com mais de um vértice, pelo mesmo argumento anterior, a resposta é sempre NÃO. Caso contrário, o problema pode ser resolvido em tempo polinomial, encontrando um emparelhamento máximo $M$ e verificando se $|M| \geq k$.

On the other hand, if the graph is disconnected, there are two possibilities. If it does not have at least one connected component with more than one vertex, by the same previous argument, the answer is always NO. Otherwise, the problem can be solved in polynomial time by finding a maximum match $M$ and checking if $|M| \geq k$.

\end{comment}

\section{Example of {\sc $2$-Disconnected Matching} transformation}

Consider the input $I$ with the two clauses $c_1 = (x \vee y \vee z)$ e $c_2 = (w \vee y \vee \overline{x})$. 

Let's build the graph $G$, $V(G) = 30m = 60$, $E(G) = 47m^2 + 24m = 236$, as described in Section \ref{subsec:transformacaoEntrada}.

We describe below the edges between $B_1$ and $B_2$. Note that in $I$, the third literal of $c_2$ is the negation of $c_1$. Therefore, the edges $\{ r_{11}l_{23}, l_{14}r_{26} \}$ must be added. In addition, the second literal of $c_1$ is the same as $c_2$. Thus, we add the edges $\{ l_{15}r_{22}, r_{12}l_{25} \}$. The rest of the literals refer to different variables, so there are no additional edges between $B_1$ and $B_2$.

We present the only two $I$ solutions for { \sc One-in-three 3SAT} and their corresponding disconnected matchings in $G$. The assignment of the variables $(w, x, y, z)$, in this order, can be either $(V, V, F, F)$, represented by the matching in Figure \ref{fig:exemploEmparelhamento1}, or $( F, F, F, V)$, in Figure \ref{fig:exemploEmparelhamento2}. For easier visualization, some edges of $B_1$ and $B_2$ are omitted, besides the complete subgraphs $H_1$ and $H_2$ and their respective $6m = 12$ saturated edges.

\begin{figure}%
        \centering
        \subfloat[]{{\includesvg[width=0.5\textwidth]{images/svg/exemplo-gadgets-indices-invertidos-emparelhamento-1-reduzido}\label{fig:exemploEmparelhamento1} }}
        \subfloat[]{{\includesvg[width=0.5\textwidth]{images/svg/exemplo-gadgets-indices-invertidos-emparelhamento-2-reduzido}\label{fig:exemploEmparelhamento2} }}
        \caption{Disconnected matching examples in the simplified clause subgraphs for the boolean expression $(x \vee y \vee z) \wedge (w \vee y \vee \overline{x})$}.%
        \label{fig:exemploEmparelhamento}
\end{figure}


\section{Proof of Theorem \ref{teo:dicotomia-emp-c-desc}}
It is simple to verify that the problem belongs to \NP, since a certificate can be a matching that induces a graph with $c$ connected components. Such matching can be verified in polynomial time. We show next that the problem is {\NPH} for some cases and {\P} for others. For $c>1$, the {\sc One-in-three 3SAT} can be reduced to {\sc $c$-Disconnected Matching} using, as an input, the transformation graph and $k = 12m + (c-2)$. Let $M$ be a matching such that $G[M]$ has $c$ connected components and $|M| \geq k$. Let's consider two $M$ partitions, contained in $U$ and $G'$. Regarding the subgraph $U$, if we consider that all edges of $E(U)$ are saturated, then $G[M]$ will have at least $c-2$ connected components. Regarding $G'$, we know that for $G'[M]$ to have the remaining $2$ connected components, the largest number of saturated edges in $G'$ must be $12m$. In total, $M$ will have exactly $12m + c - 2$ edges. Concerning the restriction on the number of connected components of $G[M]$, we conclude that $M$ is maximum and all maximum $c$-matchings in $G$ are compounded this way. For $c = 1$, Theorem \ref{teo:emp-1-desc} shows that the problem belongs to \P.

\section{Proof of Lemma \ref{lemma:c-disc-ida}}
Denote the sets of vertices $U$ by $\{ w_i^+,w_i^- \mid c_i \in C \}$ and $S$ by $\bigcup_{j=1}^{j=m} V(H_j) - U$. Let's build a matching $M$ from the solution $C'$. For each set $c_i = \{ x,y,z \}$ contained in $C'$, add the edges $w_{ix}v_x$ to $M$. Also, for each set $c_j \in C$, add the edge $w_j^+w_j^-)$. Consequently, each $H_i$ such that $c_i \notin C'$ will induce a connected component isomorphic to $K_2$ in $G[M]$, with the vertices $\{ w_i^+, w_i^- \}$, totalizing $m - q$ connected components and $2m-2q$ saturated vertices. There will also be one more connected component containing the $3q$ vertices of $\{ v_i \mid i \in \{1,\ldots,3q \} \}$ and the $5q$ vertices of $\{ W_j \mid c_j \in C - C' \}$. Thus, $M$ saturates $2m - 2q + 3q + 5q = 2m + 6q$ vertices, corresponding to $m + 3q$ edges. Also, $G[M]$ has $m - q + 1$ connected components. So, $M$ is a valid solution for the { \sc $c$-Disconnected Matching }.


\section{Proof of Lemma \ref{lemma:c-disc-volta}}
Denote the sets of vertices $U$ by $\{ w_i^+,w_i^- \mid c_i \in C \}$ and $S$ by $\bigcup_{j=1}^{j=m} V(H_j) - U$. Consider an arbitrary $c$-disconnected matching $M$, $|M| \geq k$ in $G$. Based on the graph built, we show how such matching is structured and then build a solution $C'$. Note that every edge in $G$ is either incident to a vertex of $S$ or to two vertices of $U$. Since all vertices of $S$ are connected, $G[M]$ can only have two types of connected components. 

\begin{enumerate}[(I)]
    \item A $K_2$ with $2$ vertices of $U$.
    \item A connected component that can contain any vertex, except the ones from type (I) connected components and its adjacencies.
\end{enumerate}

Given that $G[M]$ has at least $c$ connected components, then it must have at least $c-1$ connected components of type (I). For each of them, the $2$ saturated vertices are $\{ w_i^+, w_i^- \}$, that are contained in $U$. To keep these vertices in an isolated connected component, the other $3$ vertices of $W_i \cap S$ can not be saturated. So, we will not use them for the rest of the construction. In order to have $c$ connected components, it is needed at least one more. Note that, so far, we have $2c-2 = 2m - 2q$ saturated vertices, and the remaining graph has exactly $6q + 2q = 8q$ vertices. Since $M$ saturates $2k = 2m-2q$ vertices, then the other connected component, of type (II), must saturate all the remaining $8q$ vertices. Thus, there can be no more than $c$ connected components in $G[M]$ and no more than $k$ edges in $M$. Note that, for each $i \in \{1,\ldots,m \}$, the subgraph $G[W_i \cap S]$ has either $0$ or $3$ saturated vertices. If it has $3$, each vertex in $W_i \cap S$ must be matched with a vertex of $\{ v_j \mid j \{ 1,\ldots,3q \} \}$, by an edge. Such edge exists because the set $c_i$ has the element $j$. Therefore, a solution $C'$ can contain the set $c_i$ if and only if $W_i \cap S$ has $3$ saturated vertices.


\section{Proof of Theorem \ref{teo:c-disc-npc-chordal}}
We now prove, in sequence, that the problem belongs to {\NP} and is {\NPH}. Let $M$ be a $c$-disconnected matching, $|M| \geq k$. The matching $M$ serves as a certificate for the answer {\YES}, which can be verified in polynomial time, checking the size of $M$ and the number of connected components of $G[M]$. Then, the problem is in {\NP}. The Lemmas \ref{lemma:c-disc-ida} and \ref{lemma:c-disc-volta} show that a solution $C'$ for the {\sc Exact Cover by $3$-sets} corresponds to a $c$-disconnected matching $M$ and vice versa, $c = m-q+1$, $|M| = 3q+m$ in the transformation graph $G$. For this reason, { \sc $c$-Disconnected Matching } is {\NPH} and, thus, also {\NPc} even for chordal graphs.

\begin{comment}
\section{Proof of Theorem \ref{teo:c-matching-xp}}
Note that if a matching $M$ is a maximum $c$-disconnected matching of $G = (V,E)$, then $V \setminus V(M)$ contains at most $c-1$ minimal separators of $G$. Consider that $G$ has $t$ minimal separators, $\mathcal{S} = \{S_1, S_2, \ldots, S_t\}$, $t$ is polynomial in $(|V|+|E|)$. Therefore, if we analyse all subsets $S' \subseteq \mathcal{S}$ of size $k \leq c-1$ and, for each one, run the {\sc Maximum Matching} algorithm and test if the resulting matching is $c$-disconnected matching with size $\geq k$, the answer is \YES. If none of those matchings satisfy the these constraints, then the answer is \NOi. 
Note that the number of subsets $S'$ is bounded by
\[
    \sum_{i \in \{ 1,\ldots,c-1 \}} \binom{t}{i} = \sum_{i \in \{ 1,\ldots,c-1 \}} \bigO{t^i} = \bigO{t^c}
\]

Calculating a maximum matching can be done in $\bigO{|E|\sqrt{|V|}}$ and checking if the matching is a $c$-matching with $k$ edges is linear. Therefore, the whole process takes $\bigO{t^{c}|E|\sqrt{|V|}}$.
\end{comment}

\section{Proof of Theorem~\ref{teo:c-disc-interval}}
    We define $|V(G)| = n$ and $|E(G)| = m$.
    Let $(G, k, c)$ be the input to \textsc{Disconnected Matching}, $\mathcal{Q} = \langle Q_1, \dots, Q_p \rangle$ be an ordering of the maximal cliques of $G$ where each vertex in $V(G)$ occurs in consecutive elements of $\mathcal{Q}$~\cite{interval_order}, $\mathcal{S} = \{S_1, S_2, \dots, S_{p}, S_{p+1}\}$ be a set of minimal separators where $S_i = Q_i \cap Q_{i-1}$, for every $2 \leq i \leq p$, and $S_1 = S_{p+1} = \emptyset$, and $G_{i,j} = G\left[\bigcup_{i \leq \ell \leq j} Q_i \setminus (S_i \cup S_{j+1})\right]$.
    Our dynamic programming builds a table $f(i,j,c')$, where $i,j \in \{ 1,\ldots,p \}$ and $c' \in \{ 1,\ldots,c \}$, and is equal to $q$ if and only if the largest $c'$-disconnected matching of $G_{i,j}$ has $q$ edges; that is, $(G, k, c)$ is a positive instance if and only if $f(1, p, c) \geq k$.
    We define the recurrence relation for $f$ as follows:
    
    \begin{equation}
        \label{eq:interval_rec}
        f(i,j,c') = 
        \begin{cases}
            -\infty, \text{ if $c' > 1$ and $i = j$,}\\
            \beta(G_{i,j}), \text{ if $c' \in \{0, 1\}$,}\\
            \max\limits_{c_1 + c_2 = c'} \max\limits_{i \leq \ell \leq j - 1} f(i, \ell, c_1) + f(\ell+1, j, c_2), \text{ otherwise.}
        \end{cases}
    \end{equation}
    
    In the above, $\beta(K_1) = \beta(\emptyset) = -\infty$.
    If $c' \leq 1$, then, by Theorem~\ref{teo:emp-1-desc}, $\beta_{d,c}(G_{i,j}) = \beta(G_{i,j}) = f(i,j,c')$ and we are done.
    Otherwise, let $c \geq 2$, $M$ be a $c'$-disconnected matching of $G_{i,j}$ with maximum number of edges, $C_1, C_2$ be two connected components of $G[V(M)]$, and $S \subseteq V(G) \setminus V(M)$ be a non-empty minimal vertex separator between $C_1, C_2$ in $G$.
    Since $G$ is an interval graph, $S \in \mathcal{S}$, say $S = S_\ell$, and w.l.o.g. $C_1 \subset V(G_{i,\ell})$; let $c_1$ be the number of connected components in $G_{i,\ell}[V(M)]$ and $c_2$ the same quantity defined in $G_{\ell+1, j}[V(M)]$.
    By the hypothesis that $S \neq \emptyset$, we have that $|V(G_{i,\ell})|,|V(G_{\ell+1, j})| < |V(G)|$ and, by induction on the size of the input graph, we have that $f(i, \ell, c_1) = \beta_{d,c_1}(G_{i,\ell})$ and $f(\ell + 1, j, c_2) = \beta_{d,c_2}(G_{\ell+1, j})$.
    Finally, since $V(M) \cap S = \emptyset$ and $G \setminus S = G_{i,\ell} \cup G_{\ell+1, J}$, we have that $|M| = f(i, \ell, c_1) + f(\ell+1, j, c_2) \leq f(i,j,c')$ which is covered by the third case of Equation~\ref{eq:interval_rec}.
    For the converse, note that the first two cases of Equation~\ref{eq:interval_rec} are correct: (i) if $i=j$, then $G_{i,j}$ is a clique, and we can have a $c'$-disconnected matching in $G_{i,j}$ if and only if $c' \leq 1$, and (ii) if $c \leq 1$, then we are asking for a matching with an arbitrary number of connected components, which is what is returned in the second case.
    For the third case, let $\ell, c_1, c_2$ be the values that satisfy $f(i,j,c') = f(i, \ell, c_1) + f(\ell+1, j, c_2)$; $M_1$ be the corresponding $c_1$-disconnected matching in $G_{i,\ell}$, $M_2$ the $c_2$-disconnected matching in $G_{\ell+1, j}$ and $M' = M_1 \cup M_2$.
    By induction, $|M_1| = \beta_{d, c_1}(G_{i,\ell})$ and $|M_2| = \beta_{d, c_2}(G_{\ell+1, j})$, $M'$ is a $c'$-disconnected matching of $G_{i,j}$, and $f(i,j,c') = |M'| \leq |M|$.
    
    As to the running time, since we have $\bigO{n^2c}$ entries in the table and each case can be run in $\bigO{\max\{nc, m\sqrt{n}\}}$ time, it holds that the algorithm runs in polynomial time. 

\section{Proof of Theorem~\ref{teo:c-disc-tw}}

An algorithmically useful property of tree decompositions is the existence of a \emph{nice tree decomposition} that does not increase the treewidth of $G$.

\begin{definition}[Nice tree decomposition]
    A tree decomposition $\mathbb{T}$ of $G$ is said to be \emph{nice} if its tree is rooted at, say, the empty bag $r(T)$ and each of its bags is from one of the following four types:
    \begin{enumerate}
        \item \emph{Leaf node}: a leaf $x$ of $\mathbb{T}$ with $B_x = \emptyset$.
        \item \emph{Introduce vertex node}: an inner bag $x$ of $\mathbb{T}$ with one child $y$ such that $B_x \setminus B_y = \{u\}$.
        \item \emph{Forget node}: an inner bag $x$ of $\mathbb{T}$ with one child $y$ such that $B_y \setminus B_x = \{u\}$.
        \item \emph{Join node}: an inner bag $x$ of $\mathbb{T}$ with two children $y,z$ such that $B_x = B_y = B_z$.
    \end{enumerate}
\end{definition}

\begin{proof}
    We define $|V(G)| = n$ and $|E(G)| = m$.
    We suppose w.l.o.g that we are given a tree decomposition $\mathbb{T} = (T, \mathcal{B})$ of $G$ of width $t$ rooted at an empty forget node; moreover, we solve the more general optimization problem, i.e., given $(G,c)$ we determine the size of the largest $c$-disconnected matching of $G$, if one exists, in time \FPT\ on $t$.
    As usual, we describe a dynamic programming algorithm that relies on $\mathbb{T}$.
    For each node $x \in V(T)$, we construct a table $f_x(S, U, \Gamma, \ell)$ which evaluates to $\rho$ if and only if there is a (partial) solution $M_x$ with the following properties: (i) $S \subseteq B_x \cap V(M_x)$ and $G[S]$ admits a perfect matching, (ii) the vertices of $U \subseteq V(M_x) \cap B_x \setminus S$ are half-matched vertices and are going to be matched to vertices in $G \setminus G_x$, (iv) $\Gamma \in \Pi(A_x)$ is a partition of $A_x$, where $S \cup U \subseteq A_x \subseteq B_x$, and each part of $\Gamma$ corresponds to a unique connected component of $G[M_x]$ --- we say that $V(\Gamma) = A_x$ --- (iv) $G[M_x]$ has \textit{exactly} $\ell$ connected components that do not intersect $B_x$, and (v) $M_x$ has $\rho$ edges.
    If no such solution exists, we define $f_x(S, U, \Gamma, \ell) = -\infty$ and we say the state is \textit{invalid}.
    Below, we show how to compute each entry for the table for each node type.
    
    \noindent \textbf{Leaf node:} Since $B_x = \emptyset$, the only valid entry is $f_x(\emptyset, \emptyset, \{\}, 0)$, which we define to be equal to 0.
    
    \noindent \textbf{Introduce node:} Let $y$ be the child of $x$ in $T$ and $B_x = B_y \cup \{v\}$.
    We compute the table as in Equation~\ref{eq:tw_introduce}; before proceeding, we define $\Gamma(v)$ to be the block of $\Gamma$ that contains $v$ and a partition $\Gamma' \in \sift_v(\Gamma)$ if: (i) $V(\Gamma') = V(\Gamma) \setminus \{v\}$, (ii) every block in $\Gamma \setminus \Gamma(v)$ is also in $\Gamma'$, and (iii) $\Gamma'$ contains a connected refinement of $\Gamma(v) \setminus \{v\}$, i.e. there is a partition $\pi$ of $\Gamma(v) \setminus \{v\}$ that is a subset of $\Gamma'$, vertices in different blocks of $\pi$ are non-adjacent, and each block of $\pi$ has at least one neighbor of $v$.
    
    \begin{equation}
        \label{eq:tw_introduce}
        f_x(S, U, \Gamma, \ell) =
        \begin{cases}
            f_y(S, U, \Gamma, \ell), &\text{ if $v \notin V(\Gamma)$;} \\
            \max\limits_{\Gamma' \in \sift_v(\Gamma)} f_y(S, U \setminus \{v\}, \Gamma', \ell), &\text{ if $v \in U$;} \\
            \max\limits_{u \in N(v) \cap S} \max\limits_{\Gamma' \in \sift_v(\Gamma)} f_y(S \setminus \{u,v\}, U \cup \{u\},  \Gamma', \ell), &\text{ otherwise.}
        \end{cases}
    \end{equation}
    
    For the first case of the above equation, if $v \notin V(\Gamma)$ then any partial solution $M_x$ of $G_x$ represented by $(S, U, \Gamma, \ell)$ is also a solution to $G_y$ under the same constraints since $G_y = G_x \setminus \{v\}$ and $v$ is not in $V(M_x) = V(\Gamma)$.
    For the second case, let $M_x$ by the solution that corresponds to $(S, U, \Gamma, \ell)$, $C_v$ the connected component of $G[V(M_x)]$ that contains $v$, and $ \pi = \{C_1, \dots, C_q\}$ the (possibly empty) connected components of $G[C_v \setminus \{v\}]$; by definition, $C_v \cap B_x = \Gamma(v)$ is a block of $\Gamma$ and $\pi$ is a partition of $C_v$ where vertices in different blocks are non-adjacent.
    Consequently, we have that $\Gamma' = \Gamma \setminus \Gamma(v) \cup \pi$ is in $\sift_v(\Gamma)$ and $f_y(S, U \setminus \{v\}, \Gamma', \ell)$ is accounted for in the computation of the maximum, which by induction is correctly computed.
    Finally, for the third case, let $uv \in M_x$, and note that we may proceed as in the previous case: the connected components of $G[C_v \setminus \{v\}]$ induce a connected refinement $\pi$ of $\Gamma(v) \setminus \{v\}$ and $\Gamma' = \Gamma \setminus \Gamma(v) \cup \pi$ is in $\sift_v(\Gamma)$, which results in a solution of $G_y$ that corresponds to the tuple $(S \setminus \{u,v\}, U \cup \{u\}, \Gamma', \ell)$; since the maximum runs over all neighbors of $v$ in $S$ and over all partitions in $\sift_v$, our table entry is correctly computed.
    
    
    \noindent \textbf{Forget node:} Let $y$ be the child of $x$ in $T$ and $B_x = B_y \setminus \{v\}$.
    We show how to compute tables for these nodes in Equation~\ref{eq:tw_forget}, where $\Gamma^{\{u,v\}} = \Gamma \setminus \{\Gamma(u)\} \cup \{\Gamma(u) \cup \{v\}\}$, $V_{S,U}(\Gamma) = V(\Gamma) \setminus (S \cup U)$, and
    
    \begin{equation}
        \label{eq:tw_forget_aux}
        g(S, U, \Gamma, \ell, u) = \max \{f_y(S, U, \Gamma^{\{u,v\}}, \ell),\ f_y(S \cup \{u,v\}, U, \Gamma^{\{u,v\}}, \ell) + 1\}.
    \end{equation}

    \begin{equation}
        \label{eq:tw_forget}
        f_x(S, U, \Gamma, \ell) = \max
        \begin{cases}
            f_y(S, U, \Gamma, \ell) \\
            f_y(S, U, \Gamma \cup \{\{v\}\}, \ell-1) \\
            \max\limits_{u \in V(\Gamma)} f_y(S, U, \Gamma^{\{u,v\}}, \ell), \text{ if $N(v) \cap V(\Gamma) = \emptyset$;} \\
            \max\limits_{u \in N(v) \cap \gamma} g(S, U, \Gamma, \ell, u), \text{ if $\exists \gamma \in \Gamma \mid N(v) \cap V(\Gamma) \subseteq \gamma$.}
        \end{cases}
    \end{equation}
    
    Let $M_x$ be a solution to $G_x$ represented by $(S, U, \Gamma, \ell)$.
    If $v \notin V(M_x)$, then $M_x$ is a solution to $G_y$ constrained by $(S, U, \Gamma, \ell)$ and, by induction, the correctness of $f_x$ is given by the first case of Equation~\ref{eq:tw_forget}.
    Recall that, assuming $v \in V(M_x)$ implies that $N(v) \cap V(\Gamma)$ must be contained in a single block of $\Gamma$, otherwise this table entry is deemed invalid and we may safely set it to $-\infty$.
    If there is some connected component $C_v$ of $G[V(M_x)]$ that has $C_v \cap (V(\Gamma) \cup \{v\}) = \{v\}$, then it must be the case that $M_x$ is a solution of $G_y$ represented by $(S, U, \Gamma \cup \{\{v\}\}, \ell - 1)$ since $C_v \cap B_y = \{v\}$, which is the second case of the equation.
    Suppose $wv \in M_x$.
    If $\{u,v\} \subseteq C_v \cap (V(\Gamma) \cup \{v\})$, we branch our analysis on two cases:
    \begin{enumerate}
        \item For the first one, we suppose $N(v) \cap V(\Gamma) = \emptyset$ and note that $\Gamma^{\{u,v\}}(u) = C_v \cap V(\Gamma^{\{u,v\}})$, so we must have that $f_y(S, U, \Gamma^{\{u,v\}}, \ell) \neq -\infty$ is accounted for in the third case of Equation~\ref{eq:tw_forget}.
        \item Otherwise, there is some $u \in N(v) \cap V(\Gamma)$ and it must be the case that $N(v) \cap V(\Gamma) \subseteq \Gamma(u) = \gamma$. If $u = w$, then $M_x$ is a partial solution to $G_y$ represented by $(S \cup \{u,v\}, U, \Gamma^{\{u,v\}}, \ell)$, so, by induction, $f_y(S \cup \{u,v\}, U, \Gamma^{\{u,v\}}, \ell)$ is well defined, and we have one additional matched edge outside of $B_x$ than outside of $B_y$, hence the $+1$ term in Equation~\ref{eq:tw_forget_aux}.
        Finally, if $u \neq w$ and $w \notin B_x$, then we proceed as in Case 1, as shown in Equation~\ref{eq:tw_forget_aux}, but since $v$ must be in the same connected component of its neighbors, we have fewer entries to check in $f_y$.
        Either way, $u$ is accounted for in the range of the maximum in the fourth case of Equation~\ref{eq:tw_forget}.
    \end{enumerate}
    
    \noindent \textbf{Join node:} Finally, let $x$ be a join node with children $y,z$ and $B_x = B_y = B_z$. We obtain the table for these nodes according to the following recurrence relation, where $C = A \sqcup B$ is the \textit{join} between $A$ and $B$.
    
    \begin{equation}
        \label{eq:tw_join}
        f_x(S, U, \Gamma, \ell) = \max_{\substack{\ell_y + \ell_z = \ell \\ U_y \dot{\cup} U_z = V_{S,U}(\Gamma) \\ \Gamma_y \sqcup \Gamma_z = \Gamma}} f_y(S, U \cup U_y, \Gamma_y, \ell_y) + f_z(S, U \cup U_z, \Gamma_y, \ell_z)
    \end{equation}
    
    Once again, let $M_x$ be a solution to $G_x$ satisfying $(S, U, \Gamma, \ell)$ and $M_i = M_x \cap G_i$ for $i \in \{y,z\}$.
    Moreover, let $\mathcal{C}_i$ be the connected components of $G[V(M_i)]$, $\ell_i$ the number of components in $\mathcal{C}_i$ with no vertex in $B_i$, and $\Gamma_i$ the partition of $V(M_i) \cap B_i$ where each block is equal to $C \cap B_i$ for some $C \in \mathcal{C}_i$.
    Note that it must be the case that $\ell = \ell_y + \ell_z$ --- since $M_x = M_y \cup M_z$ --- and that $\Gamma = \Gamma_y \sqcup \Gamma_z$ since vertices in different connected components of $M_y$ may be in a same connected component of $M_z$, but vertices in different connected components in both solutions are not merged in a same connected component of $M_x$.
    Now, define $W_y \subseteq V_{S,U}(\Gamma)$ to be the set of vertices that are matched to a vertex of $G_y \setminus S$, let $W_z$ be defined analogously, $U_y = W_z$ and $U_z = W_y$; note that $(U_y, U_z)$ is a partition of $V_{S,U}(\Gamma)$, and that the vertices in $M_i \cap B_i$ that must be matched, but not in $G_i$, are given by $U \cup U_i$.
    As such, $M_i$ is represented by $(S, U \cup U_i, \Gamma_i, \ell_i)$ and by induction we have $f_i(S, U \cup U_i, \Gamma_i, \ell_i) = |M_i \setminus S|$, so it holds that $f_x(S, U, \Gamma, \ell) = \sum_{i \in \{y,z\}} f_i(S, U \cup U_i, \Gamma_i, \ell_i) = |M_x \setminus S|$, which is one of the terms of the maximum shown in Equation~\ref{eq:tw_join}.
    
    Recall that we may assume that our tree decomposition is rooted at a forget node $r$ with $B_r = \emptyset$; by definition, our instance $(G, k, c)$ of \textsc{Disconnected Matching} is a \YES\ instance if and only if $f_r(\emptyset, \emptyset, \{\}, c) \geq k$.
    As to the running time, we have $\bigO{2^{2t}\eta_tn}$ entries per table of our algorithm, where $\eta_t$ be the $t$-th Bell number, each of which can be computed in $\bigO{2^t\eta_{t+1}^2n}$, which is the complexity of computing a join node, so our final running time is of the other of $\bigO{8^t\eta_{t+1}^3n^2}$.
\end{proof}

==> induced.tex <==
\section{Induced and disconnected matchings}\label{sec:induced-disc}

There is a strong connection with the {\sc $k$-Induced Matching} problem, which has been proved to be NP-complete\cite{CAMERON198997}, even for some classes of graph. Below, we describe the problem and show its equivalency with {\sc $c$-Disconnected Matching} restricted to $c = k$. 
The {\sc $k$-Induced Matching} consists in, given a graph $G$ and an integer $k > 0$, decide if there exists a matching $M$, $|M| \geq k$, such that $G[M]$ is $1$-regular.

%Moreover, itremains NP-hard under substantial restrictions, for instance: for bipartite graphs of vertex degree at most 3 [27,32], linegraphs [26], planar graphs of vertex degree at most 4 [25] and even for cubic planar graphs [11]. On the other hand,polynomial-timealgorithmsforthisproblemhavebeendevelopedforweaklychordalgraphs[7],AT-freegraphs[8],circulararcgraphs[19],graphsofboundedclique-width[26]andsomeotherclassesofgraphs[

\begin{theorem}\label{teo:c-disc-induced-np-complete}
{\sc Disconnected Matching} is {\NPc} even for any of the graph classes for which the {\sc $k$-Induced Matching} is NP-complete.
\end{theorem}
\begin{comment}
\begin{proof}
The input data set for the {\sc $k$-Induced Matching} is a subset of the possible inputs from {\sc $c$-Disconnected Matching}, since these problems are equivalent when using $c = k$. Therefore, the {\sc $c$-Disconnected Matching} is NP-complete, because it is an extension of {\sc $k$-Induced matching}. Such reduction does not alter the input $G$ graph and, therefore, its properties are preserved when considering with the problem {\sc $c$-Disconnected Matching}.
\end{proof}
\end{comment}

Some classes for which the {\sc $k$-Induced Matching} problem has been proved to be {\NPc} are planar graphs of maximum degree 4\cite{10.1137/S089548019828371X}, bipartite graphs of maximum degree $3$, C4-free bipartite graphs \cite{LOZIN20027}, $r$-regular graphs for $r\geq5$, line-graphs, chair-free graphs, and Hamiltonian graphs \cite{10.1007/s00453-003-1035-4}. Thus, the {\sc Disconnected Matching} is also {\NPc} even for such classes.

%Note that, since {\sc $k$-Induced matching} is \XP, if the parameter $k$ is fixed, the problem becomes polynomial and can be solved in a simple way. One way is to check if there is a set of edges $M$, $|M| \geq k$, which induces a $1$-regular graph. Such procedure can be performed in $O(|E|^k)$, which is polynomial for a fixed $k$. A more elaborate parametrized reduction, which proves the pertinence of the problem in $W[1]$-hard for bipartite graphs, can be found in \cite{MOSER2009715}.

The treatment when setting the parameter of the {\sc $k$-Induced Matching} is simple and there is nothing to conclude about the hardness of {\sc $c$-Disconnected Matching} for a fixed $c$. We use another way to approach such problem, in Section \ref{sec:disc-c-np-complete}.
